Down the Rabbit Hole: Detecting Online Extremism, Radicalisation, and Politicised Hate Speech

Social media is a modern person's digital voice to project and engage with new ideas and mobilise communities $\unicode{x2013}$ a power shared with extremists. Given the societal risks of unvetted content-moderating algorithms for Extremism, Radicalisation, and Hate speech (ERH) detection, responsible software engineering must understand the who, what, when, where, and why such models are necessary to protect user safety and free expression. Hence, we propose and examine the unique research field of ERH context mining to unify disjoint studies. Specifically, we evaluate the start-to-finish design process from socio-technical definition-building and dataset collection strategies to technical algorithm design and performance. Our 2015-2021 51-study Systematic Literature Review (SLR) provides the first cross-examination of textual, network, and visual approaches to detecting extremist affiliation, hateful content, and radicalisation towards groups and movements. We identify consensus-driven ERH definitions and propose solutions to existing ideological and geographic biases, particularly due to the lack of research in Oceania/Australasia. Our hybridised investigation on Natural Language Processing, Community Detection, and visual-text models demonstrates the dominating performance of textual transformer-based algorithms. We conclude with vital recommendations for ERH context mining researchers and propose an uptake roadmap with guidelines for researchers, industries, and governments to enable a safer cyberspace.

==> Related-Work.tex <==
\section{Related Work}
\label{section:related-work}

Searching for \textit{Extremism}, \textit{Radicalisation}, \textit{Hate speech} (ERH) and related terms, resulted in ten literature reviews ranging from January 2011 to April 2021. Aldera et al. observed only one survey before 2011 (covering 2003 to 2011) and another in 2013, indicating the limited, exclusionary, but developing nature of studies, and literature reviews, in this ERH detection field~\cite{Aldera21_onlineextremism_textual_review}.

\textit{Extremism}, \textit{Hate Speech} and \textit{Radicalisation} were seldom delineated or elaborated within existing work, often targeting “extremism or radicalism or terrorism detection”, lemmifications of “extrem*” and “radical*” and “terror*”~\cite{Aldera21_onlineextremism_textual_review}, and esoteric terms such as \textit{propaganda}, \textit{community detection}~\cite{Aldera21_onlineextremism_textual_review, Gaikwad21_online_extremism_detection_review_tools}. Given the role of politically motivated extremists on social media, targeting “hate speech”, “polarisation” or “affiliation” within a political context--–extremist speech is often synonymous to “political hate speech” or “far-right/left political affiliation” (i.e., terms which would evade such reviews). Evidently, neither “extremism”, "radicalism"~\cite{Gaikwad21_online_extremism_detection_review_tools, Adek21_systematics_radical_extremist_review, Aldera21_onlineextremism_textual_review, agarwal2015_onlineradical_civilunrest_review} or “hate speech” oriented studies~\cite{Rini20SysLitReviewOfHateTextMining, Istaiteh20_randshatespeechlitreview} cross-reference each other as a direct result, despite 26.3\% of the data reviewed in the “hate speech” oriented review by Adek et al. encompassing hate speech in a political context (and thereby extremism) online~\cite{Adek21_systematics_radical_extremist_review}. This lack of overlap between reviews presents an industry-wide challenge for social media companies, who may oversee vital technologies for \textquote{hate speech} detection which could also work in an \textquote{extremism/radicalisation detection} model.

\subsection{Prior Algorithmic Evaluations}
Prior works' highest performing algorithmic approaches varied across years. SLRs prior to 2015 found that deep learning approaches (DLAs), such as Convolutional Neural Networks (CNN) and Long Short-Term Memory (LSTM), tended to result in 5-20\% lower F1-scores than their regular machine learning counterparts (e.g., Naïve Bayes, Support Vector Machines, and Random Forest classifiers)~\cite{Gaikwad21_online_extremism_detection_review_tools, Adek21_systematics_radical_extremist_review, Aldera21_onlineextremism_textual_review, agarwal2015_onlineradical_civilunrest_review, Rini20SysLitReviewOfHateTextMining, Istaiteh20_randshatespeechlitreview}. Transformer-based models such as Bidirectional Encoder Representations from Transformers (BERT)~\cite{bert_original_study}, reflect state-of-the-art advances in NLP via deep learning. DLA's post-2015 indicated a pivotal change towards their research as they tended to meet or exceed other non-deep models. Hence, our literature review evaluates whether these trends towards deep learning for NLP result in higher-performing models and by which metric.



\subsubsection{Domains and Criteria}\hfill\\
No review delineated or removed studies that did not use English social media data. This presents three areas of concern for researchers when attempting to compare the performance of models:
\begin{enumerate}
\item \textbf{Results may not be comparable}, if they use culture-specific lexical datasets, or language models trained on other languages.
\item \textbf{Linguistic differences and conveyance in language}---as what may be considered culturally appropriate for the majority class may appear offensive to minority groups and vice-versa.
\item \textbf{The choice of language(s) influences the distribution of target groups}---with a bias towards Islamic extremism given its global reach in both Western (predominantly ISIS) and Eastern countries (e.g., with studied online movements in the Russian Caucasus Region~\cite{mashechkin19_russia_caucasus_jihad_ml}). It is worth investigating whether Gaikwad et al.'s finding that 64\% of studies solely target \textquote{Jihadism} corroborates with our study, which targets only English data~\cite[p. 17]{Gaikwad21_online_extremism_detection_review_tools}.
\end{enumerate}


Our SLR incorporates the key approaches of dataset evaluation (including their accessibility, labels, source and target group(s)), data collection and scraping approaches, Machine Learning and Deep Learning algorithms, pre-processing techniques, research biases, and new considerations of socio-legal contexts. We conceptualise all elements for ERH context mining---consisting of a user's ideological \textit{radicalisation} to an \textit{extremist} position, and projected via \textit{hate speech}.
